Complexity Lower Bounds for Nonconvex-Strongly-Concave Min-Max Optimization

We provide a first-order oracle complexity lower bound for finding stationary points of min-max optimization problems where the objective function is smooth, nonconvex in the minimization variable, and strongly concave in the maximization variable. We establish a lower bound of $\Omega\left(\sqrt{\kappa}\epsilon^{-2}\right)$ for deterministic oracles, where $\epsilon$ defines the level of approximate stationarity and $\kappa$ is the condition number. Our analysis shows that the upper bound achieved in (Lin et al., 2020b) is optimal in the $\epsilon$ and $\kappa$ dependence up to logarithmic factors. For stochastic oracles, we provide a lower bound of $\Omega\left(\sqrt{\kappa}\epsilon^{-2} + \kappa^{1/3}\epsilon^{-4}\right)$. It suggests that there is a significant gap between the upper bound $\mathcal{O}(\kappa^3 \epsilon^{-4})$ in (Lin et al., 2020a) and our lower bound in the condition number dependence.

==> lower bound/header.tex <==
\usepackage{mathtools}
\usepackage{graphicx}
\usepackage{amsmath,amssymb,amsfonts,amsthm,amsxtra,bm}
\usepackage{amsthm}
\usepackage{xspace}
\usepackage{enumerate}
\usepackage{colortbl}
\usepackage{makecell,multirow}       % professional-quality tables
\usepackage{thmtools}  
\usepackage{xspace}
\usepackage{footnote, tablefootnote}
\usepackage{float}
\floatstyle{plaintop}
\restylefloat{table}
\usepackage{epstopdf}
\usepackage{latexsym}
\usepackage{algorithm, algorithmicx, algpseudocode}
\usepackage{todonotes}
%\usepackage{wrapfig}
%\usepackage{lipsum}
\usepackage{thmtools, thm-restate}
\usepackage{bbm}

==> lower bound/macro.tex <==
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}
\newcommand{\E}{\mathbb{E}}
\newcommand{\D}{\mathbb{D}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\SV}{\mathbb{S}}  % sample variance
\newcommand{\Cov}{\mathrm{Cov}}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\mspan}{span}
\DeclareMathOperator{\supp}{supp}
% The command can be slightly modified if you need that your defined operator uses subscripts below, as the \lim operator, in such case use \DeclareMathOperator*.
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}

\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Ber}{\mathrm{Bernoulli}}
\newcommand\innerp[2]{\left\langle #1, #2 \right\rangle}
\newcommand{\innerpc}[2]{\bigl\langle #1, #2 \bigr\rangle}
\newcommand{\innerpd}[2]{\biggl\langle #1, #2 \biggr\rangle}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}
\newcommand{\diff}{\mathrm{d}}

\newcommand{\nlsum}{\sum\nolimits}
\newcommand{\nlprod}{\prod\nolimits}

\newcommand{\bigotilde}{\tilde{\mathcal{O}}}

\newcommand{\unif}{\textnormal{unif}}
\newcommand{\cAuss}{\textnormal{N}}
\newcommand{\diag}{\textnormal{diag}}

\def\textforall{{\text{~for all~}}}
\def\textand{{\text{~and~}}}

\newcommand{\setto}{\leftarrow}

\newcommand{\cO}{\mathcal{O}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cP}{\mathsf{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\abs}[1]{\left\vert#1\right\vert}
\newcommand{\sC}{\mathbb{C}}
\newcommand{\sI}{\mathbb{I}}
\newcommand{\sN}{\mathbb{N}}
\newcommand{\pr}{\mathbb{P}}
\newcommand{\R}{\mathbb{R}}

% vectors
\newcommand{\vzero}{\boldsymbol{0}}
\newcommand{\vmu}{\boldsymbol{\mu}}
\newcommand{\vtheta}{\boldsymbol{\theta}}
\newcommand{\vb}{\boldsymbol{b}}
\newcommand{\vh}{\boldsymbol{h}}
\newcommand{\vg}{\boldsymbol{g}}

\newcommand{\ve}{\boldsymbol{e}}
\newcommand{\vv}{\boldsymbol{v}}
\newcommand{\vw}{\boldsymbol{w}}
\newcommand{\vu}{\boldsymbol{u}}
\newcommand{\vs}{\boldsymbol{s}}
\newcommand{\vx}{\boldsymbol{x}}
\newcommand{\vy}{\boldsymbol{y}}
\newcommand{\vby}{\bar{\boldsymbol{y}}}
\newcommand{\vz}{\boldsymbol{z}}
\newcommand{\half}{\frac{1}{2}}

% matrices
\newcommand{\mLambda}{\boldsymbol{\Lambda}}
\newcommand{\malpha}{\boldsymbol{\alpha}}
\newcommand{\mA}{\boldsymbol{A}}
\newcommand{\mC}{\boldsymbol{C}}
\newcommand{\mD}{\boldsymbol{D}}
\newcommand{\mF}{\boldsymbol{F}}
\newcommand{\mG}{\boldsymbol{G}}
\newcommand{\mI}{\boldsymbol{I}}
\newcommand{\mL}{\boldsymbol{L}}
\newcommand{\mQ}{\boldsymbol{Q}}
\newcommand{\mT}{\boldsymbol{T}}
\newcommand{\mU}{\boldsymbol{U}}
\newcommand{\mV}{\boldsymbol{V}}

\newcommand{\sfA}{\mathsf{A}}


\DeclareMathAlphabet{\mathsfit}{T1}{\sfdefault}{\mddefault}{\sldefault}
\SetMathAlphabet{\mathsfit}{bold}{T1}{\sfdefault}{\bfdefault}{\sldefault}

\newcommand{\rx}{\mathsfit{x}}
\newcommand{\ry}{\mathsfit{y}}
\newcommand{\rs}{\mathsfit{s}}
\newcommand{\ra}{\mathsfit{a}}
\newcommand{\rr}{\mathsfit{r}}
\newcommand{\rvy}{\boldsymbol{\mathsfit{y}}}

\makeatletter
\newcommand{\vast}{\bBigg@{3}}
\newcommand{\Vast}{\bBigg@{3.5}}
\makeatother


\newcommand{\ky}{\kappa}
\newcommand{\sigmav}{\sigma}
\newcommand{\sigmas}{\lambda}

\newcommand{\0}{\mathbf{0}}
\newcommand{\fsc}{f^{\text{sc}}}
\newcommand{\Asc}{A^{\text{sc}}}

\newcommand{\fnc}{\bar{f}^{\text{nc}}}
\newcommand{\ft}{\bar{f}^{\text{nc-sc}}}
\newcommand{\fmt}{\bar{f}_m^{\text{nc-sc}}}
\newcommand{\gbar}{\bar{g}}

\newcommand{\fft}{{f}^{\text{nc-sc}}}
\newcommand{\ffmt}{{f}_m^{\text{nc-sc}}}

\newcommand{\ffts}{{f}^{\text{nc-sc-sg}}}
\newcommand{\ffmts}{{f}_m^{\text{nc-sc-sg}}}
\newcommand{\fts}{\bar{f}^{\text{nc-sc-sg}}}
\newcommand{\fmts}{\bar{f}_m^{\text{nc-sc-sg}}}
\newcommand{\gs}{{h}^{\text{sg}}}
\newcommand{\gd}{{h}}

\newcommand{\bcX}{\cC^{T}_{R_1}}
\newcommand{\bcY}{\cC^{n(T-1)}_{nR_2}}
\newcommand{\bcZ}{\cC^{T-1}_{R_1}}

